Highly confined incident-angle-robust surface phonon polariton bound states in the continuum metasurfaces

Squeezing light into subwavelength dimensions is vital for on-chip integration of photonic technologies. One approach to overcome the diffraction limit is coupling light to material excitations, leading to polariton states. Here, we showcase how low-loss mid-infrared surface phonon polaritons enable metasurfaces supporting quasi-bound states in the continuum (qBICs) with deeply subwavelength unit cells. Utilizing 100 nm thick free-standing silicon carbide membranes, we achieve highly confined qBIC states with a unit cell volume ~ 10^4 times smaller than the diffraction limit. This results in remarkable robustness of the platform against the incident angle that is unique among qBIC systems. We also demonstrate vibrational strong coupling with a thin layer of spin-coated molecules, leveraging the small mode volume. This work introduces phononic qBICs as a novel ultra-confined nanophotonic platform, paving a way for the miniaturization of mid-infrared devices for molecular sensing and thermal radiation engineering.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
